Outlier-Robust Estimation: Hardness, Minimally Tuned Algorithms, and Applications

Nonlinear estimation in robotics and vision is typically plagued with outliers due to wrong data association, or to incorrect detections from signal processing and machine learning methods. This paper introduces two unifying formulations for outlier-robust estimation, Generalized Maximum Consensus (G-MC) and Generalized Truncated Least Squares (G-TLS), and investigates fundamental limits, practical algorithms, and applications. Our first contribution is a proof that outlier-robust estimation is inapproximable: in the worst case, it is impossible to (even approximately) find the set of outliers, even with slower-than-polynomial-time algorithms (particularly, algorithms running in quasi-polynomial time). As a second contribution, we review and extend two general-purpose algorithms. The first, Adaptive Trimming (ADAPT), is combinatorial, and is suitable for G-MC; the second, Graduated Non-Convexity (GNC), is based on homotopy methods, and is suitable for G-TLS. We extend ADAPT and GNC to the case where the user does not have prior knowledge of the inlier-noise statistics (or the statistics may vary over time) and is unable to guess a reasonable threshold to separate inliers from outliers (as the one commonly used in RANSAC). We propose the first minimally tuned algorithms for outlier rejection, that dynamically decide how to separate inliers from outliers. Our third contribution is an evaluation of the proposed algorithms on robot perception problems: mesh registration, image-based object detection (shape alignment), and pose graph optimization. ADAPT and GNC execute in real-time, are deterministic, outperform RANSAC, and are robust up to 80-90% outliers. Their minimally tuned versions also compare favorably with the state of the art, even though they do not rely on a noise bound for the inliers.

==> sections/__latexindent_temp.tex <==
%!TEX root = ../main.tex
\begin{table*}[t]
\centering\footnotesize
\setlength{\tabcolsep}{4pt}
\setlength{\extrarowheight}{3pt}
% \begin{tabular*}{lccccccc}\toprule
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} ccccccc}
\emph{Application} & \greedymc & \greedymts & \adaptmc & \adaptmts & \adaptfree & \gnc & \gncfree \\
\midrule
\scenario{Mesh Registration} & 80\% [\SI{13.71}{\second}] & 80\% [\SI{12.98}{\second}] & 80\% [\SI{14.42}{\second}]& 80\% [\SI{14.39}{\second}] & 80\% [\SI{12.36}{\second}] & 80\% [\SI{5.12}{\second}] & 80\% [\SI{10.68}{\second}]\\
\scenario{Shape Alignment} & 80\% [\SI{0.15}{\second}] & 80\% [\SI{0.15}{\second}] & 80\% [\SI{0.22}{\second}]& 80\% [\SI{0.23}{\second}] & 80\% [\SI{0.25}{\second}] & 80\% [\SI{0.03}{\second}] & 80\% [\SI{0.06}{\second}]\\
\scenario{PGO (2D)} & 60\% [\SI{5.04}{\second}] & 10\% [\SI{0.76}{\second}] & 80\% [\SI{5.04}{\second}]& 80\% [\SI{4.92}{\second}] & 60\% [\SI{5.61}{\second}] & 90\% [\SI{1.41}{\second}] & 80\% [\SI{2.17}{\second}]\\
\scenario{PGO (3D)} & 30\%[\SI{8.1}{\hour}] & 40\%[\SI{8.16}{\hour}] & 40\%[\SI{60.0}{\minute}] & 0\%[\SI{38.92}{\minute}] & 90\%[\SI{60.9}{\minute}] & 90\% [\SI{106.23}{\minute}] & 90\% [\SI{108.66}{\minute}] \\
\bottomrule\hline
\end{tabular*}
\caption{\textbf{Robustness of proposed algorithms.} Robustness to outliers and average of median running time of the proposed algorithms.}\label{table:robustness}
\vspace{-7mm}
\end{table*}

==> sections/alg-GNCBisection.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[h]\label{alg:bisection}
	\caption{\mbox{$\fitbisection$ (\gncfree's subroutine).}}
	\SetAlgoLined
	\KwIn{\mbox{Measurements $\vy_i,\;\forall i\in\measSet$;} $\noiseupbound\geq 0$; $\noiselowbound \geq 0$;\mbox{Target critical value $\gamma$}}
	\KwOut{\mbox{Initial guess for $\inthr$}}
  \BlankLine
  $a = c = \noiseupbound;\> b=\noiselowbound$\label{line:bisection-init}\;
  $(\vxx,\inset) = \gncalg(\vy, c);\> s = \fitChi(\vres(\vy_\inset,\vxx), d)$\label{line:bisection-initscore}\; 
  $e = s/\gamma$\;
  \While{$e > 1.1$ {\bf or} $e < 0.9$}{
    $c = (a+b)/2$\;
    $(\vxx,\inset) = \gncalg(\vy, c);\> s = \fitChi(\vres(\vy_\inset,\vxx), d)$\;
    \lIf{$|s/\gamma - e| < \num{1e-3}$\label{line:bisection-stop1}}{
      \KwBreak%\Return{$c$.}\;
    }
    \lElseIf{$s/\gamma > 1.1$}{
      $a = c$
    }\lElseIf{$s/\gamma > 0.9$}{
      $b = c$
    }
    \lIf{$(a-b)/a < 0.1$}{
      \KwBreak\label{line:bisection-stop2}%\Return{$c$.}
    }
    $e = s/\gamma$\;
  }
  % \mbox{$\inlierNoise \!=\! }\label{line:bisection-inlierguess-update}\;
  \Return{$\displaystyle\max_{i\; \in \; \inset}\;\{\res(\vy_{i},\vxx) \;\text{s.t.}\;\res(\vy_{i},\vxx) \!<\!c\}\label{line:bisection-return}$.}
\end{algorithm}

==> sections/alg-greedy.tex <==
%!TEX root = main.tex

% \begin{algorithm}[t]\label{alg:greedy}
% 	\caption{Greedy algorithm~\cite{nemhauser78analysis}.}
% 	\SetAlgoLined
% 	\KwIn{\prone's input.}
% 	\KwOut{Indices of measurements classified as inliers.}
% 	\BlankLine
% %	\tcc{Notation is explained in Section~\ref{sec:adaptIntro}.}
% \mbox{$\inset^0=\meas$;\!\quad$\vxx^0\in  \arg\min_{\vxx \; \in\; \calX}\;\;\|\; \vresyx{\inset^0}\;\|_\ell^2$;\!\quad$t=1$}\;
% 	\While{$\|\; \vres(\vy_{\inset^{\iteration-1}},\vxx^{\iteration-1})\;\|_\ell^2\;>\outfreethr$}{
% 		\For{$j \; \in \; \inset^{\iteration-1}$}{
% 			$\bm{z}_j \in  \arg\min_{\vxx \; \in\; \calX}\;\;\|\; \vresyx{\inset^{\iteration-1}\setminus\{j\}}\;\|_\ell^2$\;
% 		}
% 		$i \in \argmin_{j\;\in\; \inset^{\iteration-1}}\;\; \|\; \vres(\vy_{\inset^{\iteration-1}\setminus \{j\}},\bm{z}_j)\;\|_\ell^2$\;
% 		$\inset^{\iteration} =\ \inset^{\iteration-1}\setminus\{i\}$;\quad $\iteration++$\;
% 	}
% 	\Return{$\inset^{\iteration-1}$.}
% \end{algorithm}

\begin{algorithm}[t]\label{alg:greedy}
  \caption{Greedy algorithm~\cite{nemhauser78analysis}.}
  \SetAlgoLined
  \KwIn{\prone's inputs.}
  \KwOut{Indices of measurements classified as inliers.}
  \BlankLine
  $\calI\myat{0} = \meas$;\quad$t = 1$\;
  \While{$ \min_{\vxx\;\in\;\calX}\; \| \;\res(\vy_{\calI\myat{t-1}}, \vxx) \;\|_\ell^2 \;> \tau $}{ 
    $i = \argmin_{j\;\in\; \calI\myat{i-1}} \min_{\vxx\;\in\;\calX}\; \|\; \res(\vy_{\calI\myat{i-1} \setminus \{j\}}, \vxx ) \;\|_\ell^2$\;
    $\calI\myat{t} = \calI\myat{t-1}\setminus\{i\}$\;
  }
  \Return{$\calI\myat{t}$.}
\end{algorithm}


==> sections/failure-greedy.tex <==
%!TEX root = ../main.tex


\subsection{Limitation of the greedy algorithm}\label{sec:app-failure-greedy}
A failure mode of the causal greedy is that it can never correct mistakes made in earlier steps.
An example where this behavior leads to a wrong estimate (while \adapt is able to correct the mistake) is shown in Fig.~\ref{fig:greedy_failure}.
The example depict a line fitting problem where three points (1, 3 and 5) are inliers and two points (2 and 4) are outliers.
% The variable we want to estimate $\vxx$ represent the angular coefficient and the intercept of the line.
Let us first follow the execution of the greedy algorithm.
The \greedy initialize its initial estimate $\vxx\myat{0}$ using all available measurements (iteration 0).
In the first iteration, the \greedy removes point \num{1} (an inlier) permanently from the set of estimated inliers because it has the biggest residual, and computes the new estimate $\vxx\myat{1}$ using all remaining points ($2,\ldots,5$).
In the second iteration, removes permanently point \num{5} (another inlier) from the set of estimated inliers and computes the new estimate $\vxx\myat{2}$.
In the last iteration, the last ground truth inlier (point \num{3}) has the biggest residual, therefore the greedy algorithm removes it from set of estimated inliers converging to the set of two outliers as the estimated set of inliers.
Since the fit of the two points is below the inlier threshold, it stops.
\adapt on the other hand initialize its estimate using all available measurements and set the inlier threshold $\inthr\myat{0} = \sqrt{0.99}\cdot\res(\vy_1,\vxx\myat{0})$ since \num{1} is the point with the biggest residual.
In the first iteration, \adapt removes all points above the current threshold, in our example it removes point \num{1} (an inlier) and \num{2} (an outlier) from the set of estimated inliers as their residuals is bigger than $\inthr\myat{0}$.
It than computes the new estimate $\vxx\myat{1}$ and decrease the inlier threshold to $\inthr\myat{1} = \sqrt{0.99}\cdot\res(\vy_4,\vxx\myat{1})$ (point \num{4} has the biggest residual).
In the second iteration point \num{1} is within the current inlier threshold $\inthr\myat{1}$ so it is included in the set of estimated inliers while the two outliers (point \num{2} and point \num{4}) are above the threshold, in other words it recovered from a wrong choice made in past iterations, and the new estimate $\vxx\myat{2}$ is computed using the correct set of inliers thus estimating the correct line.
\adapt then decrease the inlier threshold $\epsilon\myat{2}$ to a value that is below the $\minnoisebound$ and stops.

==> sections/fig-alg.tex <==
%!TEX root = main.tex

\begin{figure}[t]
	\begin{center}
	\begin{minipage}{\textwidth}
	\hspace{-0.2cm}
	\includegraphics[width=.5\columnwidth]{FBT-exec} 
	\end{minipage}
\caption{Visualization of a few iterations of \name (see notation introduced in Section~\ref{sec:algorithms}).  At the beginning of each iteration, the forward step of \name builds a set $\selSet$ of seemingly outlying measurements.  It does so until the ``outlier-free'' performance bound $\perfBudgMin_{\grSet\setminus \selSet}$ is met (green, dashed line).  Then, the backward step of \name reinstates measurements in $\selSet$ as inliers.  It does so until the ``outlier-free'' bound is violated by an addititive factor $a(i)r(\emptyset)$ (orange, dotted line), during the $i$-th iteration. The process continuous until concensus is achieved.
	 \label{fig:FBT-exec}}
	\vspace{-8mm} 
	\end{center}
\end{figure}

==> sections/fig-failure.tex <==
%!TEX root = ../main.tex

\begin{figure}[t]
  \vspace{2mm} % To align with text
  \begin{center}
  	\begin{minipage}{\columnwidth}
  	\begin{tabular}{cc}%
  		\hspace{-3mm}
  		\begin{minipage}{\mpColFour}%
  			\centering%
  			\includegraphics[width=\columnwidth]{failure/greedy/simple/greedy_0.pdf}
  		\end{minipage}
  		& \mpMidSpaceFour
  		\begin{minipage}{\mpColFour}%
  			\centering%
        \includegraphics[width=\columnwidth]{failure/greedy/simple/adapt_0.pdf}
      \end{minipage}
      \\ \hspace{-3mm} %--------------
      \begin{minipage}{\mpColFour}%
  			\centering%
  			\includegraphics[width=\columnwidth]{failure/greedy/simple/greedy_1.pdf}
  		\end{minipage}
  		& \mpMidSpaceFour
  		\begin{minipage}{\mpColFour}%
  			\centering%
        \includegraphics[width=\columnwidth]{failure/greedy/simple/adapt_1.pdf}
      \end{minipage}
      \\ \hspace{-3mm} %--------------
      \begin{minipage}{\mpColFour}%
  			\centering%
  			\includegraphics[width=\columnwidth]{failure/greedy/simple/greedy_2.pdf}
  		\end{minipage}
  		& \mpMidSpaceFour
  		\begin{minipage}{\mpColFour}%
  			\centering%
        \includegraphics[width=\columnwidth]{failure/greedy/simple/adapt_2.pdf}
      \end{minipage}
      \\ \hspace{-3mm} %--------------
      \begin{minipage}{\mpColFour}%
  			\centering%
  			\includegraphics[width=\columnwidth]{failure/greedy/simple/greedy_3.pdf}
  		\end{minipage}
  		& \mpMidSpaceFour
  		\begin{minipage}{\mpColFour}%
  			\centering%
        \includegraphics[width=\columnwidth]{failure/greedy/simple/adapt_3.pdf}
      \end{minipage}
  	\end{tabular}
  \end{minipage}
  \begin{minipage}{\textwidth}
  \end{minipage}
  \vspace{-3mm} 
  \caption{Example of failure of the greedy algorithm on a line fitting problem. Point 1,3 and 5 are noiseless inliers, 2 and 4 are outliers. 
  Green dots represent inliers correctly classified as so (True Positive), yellow dots represent outliers wrongly classified as inliers (False Positive), blue dots represent inliers wrongly classified as outliers (False Negative) and red dots represent outliers correctly classified as outliers (True Negative).\label{fig:greedy_failure}}  
\end{center}
% \vspace{-5mm} 
\end{figure}


==> sections/fig-introSummary3x2.tex <==
%!TEX root = main.tex

\newcommand{\introFigTitleWidth}{0.2cm}
\newcommand{\introFigColWidth}{4cm}
\newcommand{\introFigSpacing}{\hspace{-2mm}}
\newcommand{\intoFigNameSpacing}{}

\begin{figure}[t!] 
\begin{center}
\begin{minipage}{\textwidth}
  \begin{tabular}{p{\introFigTitleWidth}p{\introFigColWidth}p{\introFigColWidth}}%
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}{\introFigTitleWidth}%
		\rotatebox{90}{Pose Graph\vspace{-4cm}}
  \end{minipage}
  &
  \begin{minipage}{\introFigColWidth}%
    \centering%
    \includegraphics[width=0.75\columnwidth]{overview/sphere_dcs.png} \hspace{-8mm}\\
    (a) \dcs
  \end{minipage}
  & \introFigSpacing
  \begin{minipage}{\introFigColWidth}%
    \centering%
    \includegraphics[width=\columnwidth]{overview/sphere_gnc.png} \hspace{-8mm}\\
    (b) \gnc
  \end{minipage}
  \\[3.5cm] % -----------------------------------------------------------
  \begin{minipage}{0.3cm}%
		\rotatebox{90}{Shape Alignment\hspace{-1.8cm}}
  \end{minipage}
  & 
  \begin{minipage}{\introFigColWidth}%
    \vspace{-1.4cm}
    \centering%
    \includegraphics[width=\columnwidth]{overview/shape_ransac.png}\intoFigNameSpacing\\
    (b) \ransac
  \end{minipage}
  & \introFigSpacing 
  \begin{minipage}{\introFigColWidth}%
    \vspace{-1.4cm}
    \centering%
    \includegraphics[width=\columnwidth]{overview/shape_gnc.png}\intoFigNameSpacing\\
      (b) \gnc
  \end{minipage}
  \\[2.5cm] % ----------------------------------------------------------
  \begin{minipage}{0.3cm}%
		\rotatebox{90}{Mesh Registration\hspace{-2cm}}
  \end{minipage}
  &
  \begin{minipage}{\introFigColWidth}%
    \vspace{-1.6cm}
    \centering%
    \includegraphics[width=\columnwidth]{overview/mesh_aeroplane_ransac.pdf}\intoFigNameSpacing\\
      (b) \ransac
  \end{minipage}
  & \introFigSpacing
  \begin{minipage}{\introFigColWidth}%
    \vspace{-1.6cm}
    \centering%
    \includegraphics[width=\columnwidth]{overview/mesh_aeroplane_adapt.pdf}\intoFigNameSpacing\\
      (b) \gnc
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \end{tabular}
\end{minipage}
\vspace{1mm} 
\caption{{\bf Summary.} Qualitative performance of the proposed algorithm against the state-of-the-art: (a) \DCS on \scenario{Sphere}, (b) \gnc on \scenario{Sphere} (c) \ransac on \scenario{FG3DCar} (d) \gncfree on \scenario{FG3DCar} (e) \ransac on \scenario{PASCAL+} dataset (f) \adapt on \scenario{PASCAL+} \label{fig:introSummary}.} 
\vspace{-9mm} 
\end{center}
\end{figure}

==> sections/fig-robustCost.tex <==
%!TEX root = main.tex

\begin{figure}[t!] 
	\begin{center}
	\begin{minipage}{\textwidth}
	\begin{tabular}{cc}%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\hspace{-4mm}
			\begin{minipage}{\mpColFour}%
			\centering%
			\includegraphics[width=\columnwidth]{gray}
			\end{minipage}
		& \mpMidSpaceFour
			\begin{minipage}{\mpColFour}%
			\centering%
			\includegraphics[width=\columnwidth]{gray} 
			\end{minipage}
		\end{tabular}
	\end{minipage}
	\vspace{-3mm} 
	\caption{{\bf M-estimation as a continuous approximation to maximum consensus.}\label{fig:robustCost}} 
	\vspace{-9mm} 
	\end{center}
\end{figure}


==> sections/figures/fig-greedy_vs_adapt.tex <==
\begin{figure}[h]
	\begin{center}
  \centering%
  \includegraphics[width=1.0\columnwidth]{failure/greedy/Failure}
  \caption{Example of failure of the greedy algorithm on a line fitting problem. Point 1,3 and 5 are noiseless inliers, 2 and 4 are outliers. 
  Green dots represent inliers correctly classified as so (True Positive), yellow dots represent outliers wrongly classified as inliers (False Positive), blue dots represent inliers wrongly classified as outliers (False Negative) and red dots represent outliers correctly classified as outliers (True Negative).\label{fig:greedy_failure}} 
\end{center}
\end{figure}

==> sections/formulation-old.tex <==
%!TEX root = ../main.tex

\section{Outlier-Robust Estimation:\\ Generalized \maxcon and \tls  Formulations}
\label{sec:formulation}

%
Sections~\ref{subsec:prone} and~\ref{subsec:prtwo}
 present {\proneLong} (\prone) and {\prtwoLong} (\prtwo) formulations. 
 % (Section~\ref{subsec:prone}, and Section~\ref{subsec:prtwo}, respectively).  
%\prone, introduced in Section~\ref{subsec:prone}, encapsulates \emph{maximum consensus} (\maxcon) and \emph{minimally trimmed squares} (\mts).  \prtwo, presented in Section~\ref{subsec:prtwo}, generalizes \emph{truncated least squares} (\tls). 
Section~\ref{subsec:mle_interpretation} gives \prone's and \prtwo's probabilistic justification % with {maximum likelihood estimation} (\mle) 
(Propositions~\ref{th:mle_for_mc}-\ref{th:mle_for_tls}).
%
Section~\ref{subsec:relationship}
provides conditions for \prone and \prtwo to be {equivalent} (Theorem~\ref{th:relationship}).
%  and Proposition~\ref{th:inf-GMC-GTLS-equiv}).  
 \optional{Finally, we demonstrate the conditions can be violated, with \prtwo rejecting more measurements than \prone  as outliers (Example~\ref{ex:tls_vs_mts} in Section~\ref{subsec:relationship}). Therein,  we also show \prtwo may lead to more accurate estimates than \prone, even when \prtwo rejects more measurements as outliers.}{}

We use the following notation:
\begin{itemize}
	\item $\vxxtrue$ is the true value of $\vxx$ we want to estimate; % (noise- and outlier-free)
	\item $\outsettrue$ is the true set of outliers;
	\item $\vresyx{\inset}\triangleq \left[ \resyx{i}\right]_{i\in\inset}$, for any $\inset\subseteq \measSet$; \ie $\vresyx{\inset}$ is the vector of residuals for the measurements $i \in \inset$.
\end{itemize}

\subsection{\proneLong \emph{(\prone)}}\label{subsec:prone}
We present a generalized maximum consensus formulation.

\begin{problem}[\proneLong (\prone)]\label{pr:main_1}  
Find an estimate $\vxx$ by solving the combinatorial problem %mixed integer program 
\beq 
%\min_{\vxx \;\in \;\calX}  \;\; \min_{\outset \; \subseteq \; \measSet}
\optmshort{\min} \quad |\outset| \;\;\;\text{\emph{s.t.}}\;\;\;  \|\; \vresyx{\measSet\setminus \outset} \;\|_\ell^2 \;\leq \outfreethr, \label{eq:main_1}
\eeq
where $\outfreethr \geq 0$ is 
a \emph{given} \inthrlong, 
and $\|\cdot\|_\ell$ denotes a generic vector norm \emph{(}in this paper, $\ell \in \{2, \infty\}$\emph{)}.
%\emph{given} type of norm \emph{(in this paper, $\ell \in \{2, \infty\}$)}.
\end{problem}

Since the true number of outliers is unknown, 
\prone rejects the least amount of measurements such that the remaining ones appear as inliers.
% at an estimate $\vxx$. 
In \eqone, $\outset$ is the set of
measurements classified as outliers; % (specifically, their indices);
% (in particular, $\outset$ is the set of indices of these measurements), 
 correspondingly, $\measSet\setminus \outset$ is the set of
%measurements to be kept as 
 inliers.
%is the indices of 
%the remaining measurements, classified as inliers. 
A choice of inliers $\measSet\setminus \outset$ is feasible only if there exists an $\vxx$ such that the cumulative residual error $\|\;\vresyx{\measSet\setminus \outset} \;\|_\ell$ satisfies the \inthrlong $\outfreethr$ (enforced by the constraint).
%, per the condition $\|\;\vresyx{\measSet\setminus \outset} \;\|_\ell \;\leq \outfreethr$ in \eqone.  
%As such, $\vxx$ is considered outlier-robust.

\prone generalizes existing combinatorial outlier-rejection formulations.
In particular, depending on the choice of $\ell$ and $\outfreethr$ in \eqone, \prone is equivalent to \maxconLong (\maxcon) 
or \mtsLong (\mts):

\begin{itemize}
\item \myParagraph{\maxcon as \prone} If $\ell=+\infty$ and $\outfreethr = \inthr^2$ in \eqone, then \prone is equivalent to \maxcon (eq.~\eqref{eq:maxConsensus}), since $\|\; \vresyx{\measSet\setminus \outset} \;\|_\infty\;\leq \inthr^2$ implies $\resyx{i} \leq \inthr$, $\forall \; i\in \MminusO$.  
%Thereby, by minimizing $\outset$'s cardinality, \prone maximizes 
%the cardinality of $\MminusO$, \ie 
%the number of measurements $\vy_i$ such that $\resyx{i} \leq \inthr$, which is the same objective as that of \maxcon.

\item \myParagraph{\mts as \prone} If $\ell=2$ in \eqone, then \prone is equivalent to the \mts~\cite{Rousseeuw87book,Tzoumas19tr-adapt} formulation
 \bea\label{eq:mts}
\optmshort{\min}\quad |\outset|  \;\;\;\text{s.t.}\;\;\; \textstyle\sumAllPointsIn{\measSet\setminus \outset} \; \resSqyx{i} \leq \outfreethr,
\eea
since $\|\; \vresyx{\measSet\setminus \outset} \;\|_2^2\; =\sumAllPointsIn{\measSet\setminus \outset} \; \resSqyx{i}$.
\end{itemize}
% All in all, \prone is a  mixed integer formulation for outlier-robust estimation, unifying the traditional formulations of maximum consensus and minimally trimmed squares.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\prtwoLong \emph{(\prtwo)}} \label{subsec:prtwo}

We present a second formulation that generalizes truncated least squares in M-estimation~\cite{Lajoie19ral-DCGM,Yang19iccv-QUASAR}.

\begin{problem}[\prtwoLong (\prtwo)]\label{pr:main_2}  
Find an estimate $\vxx$ by solving the program
\beq 
%\min_{\vxx \;\in \;\calX}  \;\; \min_{\outset \; \subseteq \; \measSet}
\optmshort{\min} \quad  \|\; \vresyx{\measSet\setminus \outset} \;\|_\ell^2 \; + \; \lag |\outset|, \label{eq:main_2}
\eeq
where $\|\cdot\|_\ell$ is a generic vector norm \emph{(}in this paper, $\ell \in \{2, {\infty}\}$\emph{)},
%$\ell$ is a \emph{given} type of norm  \emph{(in this paper, $\ell= 2$)}, 
and $\lag > 0$ is a \emph{given} penalty coefficient. %function (real valued).
\end{problem}

\prtwo looks for an outlier-robust estimate $\vxx$ by separating the measurements into inliers and outliers such that the former are penalized with their cumulative residual error $\|\; \vresyx{\measSet\setminus \outset} \;\|_\ell^2$, and the latter with their weighted cardinality $\lag |\outset|$.  
\optional{Intuitively, if the contribution of  measurement $i$ to the cumulative residual error is more than $\lag$, then the measurement will be classified as an outlier (instead of an inlier).  Evidently, if $\lag \leq 0$, then \prtwo classifies all measurements as outliers, and, trivially, $\|\; \vresyx{\measSet\setminus \outset} \;\|_\ell^2 = 0$; therefore, we generally set $\lag > 0$ in \eqtwo.  Moreover,}{}
For appropriate choices of $\lag$, \prtwo is equivalent to truncated least squares (\tls) or standard least squares (\ls):

\begin{itemize}
\item \myParagraph{\tls as \prtwo}  If $\ell=2$ and $\lag=\inthr^2$, then \prtwo becomes
\beq 
%\min_{\vxx \;\in \;\calX}  \;\; \min_{\outset \; \subseteq \; \measSet}
\optmshort{\min} \quad   \sumAllPointsIn{\MminusO}\resSqyx{i} \; + \; \sumAllPointsIn{\outset}\inthr^2 , \label{eq:main_2'}
\eeq
which is equivalent to the \tls formulation~\cite{Lajoie19ral-DCGM,Yang20arxiv-teaser,Yang19iccv-QUASAR}, commonly written using auxiliary binary variables $w_i$ as\!
\begin{equation}\label{eq:tls}
\min_{\vxx \;\in \;\calX}\;\;\;  \sumAllPointsIn{\meas}\; \min_{w_i \;\in\; \{0,1\}} \;\left[w_i\;\resSqyx{i}  +  (1-w_i)\;\inthr^2\right].
\end{equation}

\item \myParagraph{\ls as \prtwo}  If $\ell=2$ and $\lag=+\infty$, then, \prtwo becomes the least squares formulation in eq.~\eqref{eq:leastSquares}.
\end{itemize}

\subsection{\prone and \prtwo as likelihood estimation optimization}\label{subsec:mle_interpretation}

We provide a probabilistic justification for the \prone and \prtwo formulations, under the standard assumption of independent noise across the measurements.

\omitted{Our derivations in the rest of this section takes the standard assumption of independent measurement noise.}

\begin{assumption}[Independent noise]\label{ass:independence}
	If $i\neq j$, for any $i,j\in \measSet$, then $\resyx{i}$ and $\resyx{j}$ are independent random variables.
\end{assumption}

\omitted{Assumption~\ref{ass:independence} implies the joint probability density of the residuals equals the product of each residual's probability density; more formally, for any $\inset\subseteq \measSet$,
\begin{equation*}
d(\vresyx{\inset})=\prod_{i\; \in \; \inset} \;d(\resyx{i}),
\end{equation*}
where $d(\cdot)$ denotes a probability density.}


The results below provide a probabilistic grounding for two \prone's instances, 
\maxconLong (\maxcon) and \mtsLong (\mts), via likelihood estimation. % (\mle).

\begin{proposition}[Uniform inlier distribution leads to \maxcon]\label{th:mle_for_mc}
If $\res(\vy_{i}, \vxxtrue)$ is uniformly distributed with support  $[0,\inthr]$ for any $i \in \measSet \setminus \outsettrue$,  then \maxcon is equivalent to
\begin{equation}\label{eq:mle_for_mc}
%\min_{\vxx \;\in \;\calX} \;\; \min_{\outset \; \subseteq \; \measSet} 
\optmshort{\min}\quad |\outset| \;\;\;\emph{\text{s.t.}}\;\;\prod_{i\; \in \; \MminusO} u(\resyx{i})\;\geq \frac{1}{\inthr^{{|\MminusO|}}},
\end{equation} 
where $u(\res)$ is the probability density function of the uniform distribution with support $[0,\inthr]$.
\end{proposition}

The optimization in eq.~\eqref{eq:mle_for_mc} is a \emph{likelihood-constrained} estimation:
 % over the largest set of measurements appearing as \emph{inliers} at an estimate $\vxx$.  
%In more detail, since the number of outliers is unknown, eq.~\eqref{eq:mle_for_mc} rejects the least number of measurements such that the remaining measurements appear as inliers at an estimate $\vxx$.  
eq.~\eqref{eq:mle_for_mc} finds an $\vxx$ such that the joint likelihood of the inliers is at least $1/\inthr^{|\MminusO|}$.  Satisfying this bound is equivalent to maximizing the inliers' joint probability density.
\optional{\red{either the probability density equals $1/\inthr^{|\MminusO|}$, when all measurements in $\MminusO$ appear as inliers (\ie when $\resyx{i} \leq \inthr$ for all $i \in \MminusO$), or it equals $0$, otherwise.}}{} 
\optional{Overall, eq.~\eqref{eq:mle_for_mc} is an \mle formulation, and \maxcon is equivalent to it.}{}

\begin{proposition}[Folded Normal inlier distribution leads to \mts]\label{th:mle_for_mts}
If $\res(\vy_{i}, \vxxtrue)$ follows a folded Normal random distribution for any $i \in \measSet \setminus \outsettrue$, then \mts is  equivalent to
\begin{equation}\label{eq:mle_for_mts}
%\min_{\vxx \;\in \;\calX} \;\; \min_{\outset \; \subseteq \; \measSet} 
\optmshort{\min} \quad |\outset| \;\;\;\emph{\text{s.t.}}\;\;\prod_{i\; \in \; \MminusO} g(\resyx{i}) \geq 
%\frac{1}{(2\inthr)^{{|\MminusO|}}}
\frac{e^{-\frac{\outfreethrintro}{2}}}{(\pi/2)^{\frac{|\MminusO|}{2}}},
\end{equation}
where {$g(\res)\triangleq \sqrt{2/\pi}\; \exp(-\res^2/2)$} is the density of a Normal distribution constrained on the non-negative axis $(\res\geq 0)$.
\end{proposition}

Proposition~\ref{th:mle_for_mts} implies \mts is equivalent to a likelihood-constrained estimation, where the inliers follow a folded Normal distribution (in contrast to Proposition~\ref{th:mle_for_mc} where the inliers are uniformly distributed).  
\omitted{In other words, \mts looks for an estimate with a large set of inliers that best fit a folded Normal distribution.} 
\optional{The equivalence is evident once we consider the $-\log(\cdot)$ of both the sides of  the inequality in eq.~\eqref{eq:mle_for_mts}.} 

%\LC{not worth mentioning unless you add a theorem in the appendix about this: Moreover, \prone is equivalent to \mle for additional values of $\ell$ in \eqone: for example, if $\ell=1$, a common norm type in linear coding theory~\cite{Candes05tit}, then \prone is equivalent to \mle when the inliers are assumed of exponential distribution.  Such $\ell$-instances are outside the scope of applications in this paper.} 

Similarly, we show that an instance of \prtwo, truncated least squares, 
can be interpreted as a maximum likelihood estimator (\tls).  Assuming a known number of outliers, we first show \tls connects to the folded Normal distribution similarly to \mts, with respect to the inliers probability density (Proposition~\ref{th:mle_for_tls}). Then, we provide a broader characterization, connecting \tls to the Weibull distribution
 (Proposition~\ref{th:mle_for_tls-weibull}).

\begin{proposition}[Folded Normal distribution and known number of outliers lead to \tls]\label{th:mle_for_tls}
	Assume $\res(\vy_{i}, \vxxtrue)\leq \inthr$ for any $i \in \measSet \setminus \outsettrue$ and $|\outsettrue|$ is known.  If $\res(\vy_{i}, \vxxtrue)$ is a folded Normal random variable for each $i \in \MminusO$, then \tls is equivalent to 
	the cardinality-constrained maximum likelihood estimator
	\begin{equation}\label{eq:mle_for_tls}
	\max_{\substack{ \vxx \;\in \;\calX \\ \outset \; \subseteq \; \measSet,\; |\outset|\;=|\outsettrue|}}\quad\prod_{i\;\in\;\MminusO} \; g(\resyx{i}).
	\end{equation}
\end{proposition}

\begin{proposition}[Weibull distribution leads to \tls]\label{th:mle_for_tls-weibull}
Assume $\res(\vy_{i}, \vxxtrue)\leq \inthr$ for any $i \in \measSet \setminus \outsettrue$.  If $\res(\vy_{i}, \vxxtrue)$ is a Weibull random variable for each $i \in \measSet$, with \emph{cumulative probability distribution} $\mathrm{Weib}(\res)\triangleq 1-\exp{(-\res^2/2)}$, then \tls is equivalent to 
the maximum likelihood estimator
\begin{equation}\label{eq:mle_for_tls-weibull}
{\optmshort{\max}}\;\;\prod_{i\;\in\;\MminusO} \; \left[1-\mathrm{Weib}(\resyx{i})\right] \; \prod_{i\; \in \; \outset}\;  \left[1-\mathrm{Weib}(\inthr)\right].
\end{equation}
\end{proposition}
Broadly speaking, the Weibull distribution is commonly used in statistics to model the probability of an outcome's \emph{failure} when the failure depends on sub-constituent failures: \eg a chain breaks if any of its rings break~\cite{Weibull1951applmech-weibull}.  
Similarly, an outlier-robust estimate ``breaks'' if measurements are misclassified as inliers instead of outliers and vice versa, and if the inliers' residuals are unnecessarily large.
Eq.~\eqref{eq:mle_for_tls-weibull} grounds this intuition on a probabilistic framework that models both the inliers' and outliers' effect:\footnote{In stark contrast to eq.~\eqref{eq:mle_for_tls-weibull} for \tls, the interpretations of \maxcon and \mts in eq.~\eqref{eq:mle_for_mc} and eq.~\eqref{eq:mle_for_mts} do not probabilistically model the outliers' effect.} 
\begin{itemize}
	\item if a measurement $i$ is classified as an outlier ($i \in \outset$), then $1-\mathrm{Weib}(\inthr)$ models the probability of a \emph{successful} estimation given that $i$'s residual is \emph{at least} $\inthr$;
	\item if a measurement $i$ is classified as an inlier ($i \in \MminusO$), then $1-\mathrm{Weib}(\resyx{i})$ models the probability of a \emph{successful} estimation given that $i$'s residual is at least $\resyx{i}$ \emph{but not more than} $\inthr$: indeed, if $\resyx{i}>\inthr$, then eq.~\eqref{eq:mle_for_tls-weibull} classifies $i$ as an outlier, so to maximize the joint probability likelihood, since $1-\mathrm{Weib}(\resyx{i})<1-\mathrm{Weib}(\inthr)$. Therefore, for all $i\in \MminusO$, $\resyx{i} \leq \inthr$.
\end{itemize} 
In summary, eq.~\eqref{eq:mle_for_tls-weibull} aims to find $(\vxx, \outset)$ that maximize the probability of the estimator's success, and, particularly, it does so by forcing the inliers' $\resyx{i}$ to be as small as possible, since indeed $1-\mathrm{Weib}(\resyx{i})\rightarrow 1$ when $\resyx{i}\rightarrow 0$.

%%%%OLD
%states \tls is equivalent to maximum likelihood estimation where the joint probability density of all measurements breaks into (a) a group of inliers, $\MminusO$, where each inlier $i \in \MminusO$ has the folded Normal probability density $g(\resyx{i})$, and (b) a group of outliers, $\outset$, where each outlier $i \in \outset$ also has folded Normal probability density but is assumed to always have $\resyx{i} =\inthr$. 
%\optional{In effect, each outlier $i \in \outset$ discounts the inliers' joint density in eq.~\eqref{eq:mle_for_tls} with the same amount.  This is necessary for eq.~\eqref{eq:mle_for_tls} to find an outlier-robust $\vxx$.  Indeed, if we assume the contrary, \ie that outliers with larger residuals can discount more, then eq.~\eqref{eq:mle_for_tls} would look for an $\vxx$ making the outliers' residuals as small as possible;
% (since eq.~\eqref{eq:m≥le_for_tls} aims to maximize the joint probability density of all measurements); 
% but at the true $\vxxtrue$, the true outliers' residuals are large.}{}
%\omitted{The fact that eq.~\eqref{eq:mle_for_tls} considers the joint probability density of \emph{all} measurements is
%\omitted{: both the classified as inliers (measurements in $\MminusO$), and the classified as outliers  (measurements in $\outset$).  This is} in contrast to the likelihood-constrained formulations in eq.~\eqref{eq:mle_for_mc} and eq.~\eqref{eq:mle_for_mts}, where only the joint probability density of the inliers is considered.}

\optional{
The proof of Proposition~\ref{th:mle_for_tls}  relies on taking the $-\log(\cdot)$ of the objective function in eq.~\eqref{eq:mle_for_tls}, which then results to \tls.}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relationship of \prone and \prtwo}\label{subsec:relationship}

The following theorem states that \prone and \prtwo may compute two different sets of outliers, 
and \red{\tls in particular may reject more measurements as outliers than \mts.}  

\begin{theorem}[Relationship of \prone and \prtwo]\label{th:relationship}
Denote by:
\begin{itemize}
	\item $(\vxx_\prone, \outset_\prone)$ a solution to \prone;
%	 such that, among all other optimal solutions $(\vxx,\outset)$ to \prone, $\|\;\res(\vy_{\measSet\setminus \outset_\prone}, \vxx_\prone)\;\|_\ell^2$ is minimal;
%	\item $\outfreethr_\prone \triangleq \|\;\res(\vy_{\measSet\setminus \outset_\prone}, \vxx_\prone)\;\|_\ell^2$; 
	\item $(\vxx_\prtwo, \outset_\prtwo)$  a solution to \prtwo;	
%	\item $\res_{\prtwo}\triangleq \|\;\res(\vy_{\measSet\setminus \outset_\prtwo}, \vxx_\prtwo)\;\|_\ell$; \ie $\res_{\prtwo}$ is the optimal value of 
	\item  $r^2_\prtwo(\lag)$
	the cumulative residual error of the measurements classified as inliers at $(\vxx_\prtwo, \outset_\prtwo)$, \ie $r^2_\prtwo(\lag)\triangleq \|\res(\vy_{\measSet\setminus \outset_\prtwo}, \vxx_\prtwo)\|_\ell^2$;
	\item $f_\prtwo(\lag)$ the optimal value of \prtwo, \ie $f_\prtwo(\lag)\triangleq r^2_\prtwo(\lag)+\lag |\outset_\prtwo|$.
\end{itemize}
\smallskip
Then, for any $\lag, \outfreethr >0$,
%\beq\label{eq:equivalency}
%${f_\prtwo(\lag)}-\lag |\outset_\prone| \;\leq {\outfreethr}$,
%\eeq
%If eq.~\eqref{eq:equivalency} holds with equality,
%then \emph{($\vxx_\prone, \outset_\prone$)} is a solution also to \prtwo.  
%and
\begin{itemize}
	\item if $\outfreethr = r^2_\prtwo(\lag)$, then  $|\outset_\prtwo|\; = |\outset_\prone|$, and, in particular, $(\vxx_\prtwo, \outset_\prtwo)$ is also a solution to \prone; 
	\item if $\outfreethr > r^2_\prtwo(\lag)$, then $|\outset_\prtwo|\;\geq |\outset_\prone|$;
	\item if $\outfreethr < r^2_\prtwo(\lag)$, then $|\outset_\prtwo|\; < |\outset_\prone|$, and it is impossible for \prone and \prtwo to share solutions.
\end{itemize}
%Generally, if $\ell=2$, then $|\outset_\prtwo|\;\geq  |\outset_\prone|$ and $\|\res(\vy_{\measSet\setminus \outset_\prtwo}, \vxx_\prtwo)\|_\ell^2 \; \leq \outfreethr_\prone$.
% , while if $\ell=+\infty$, then equality holds if $\nu \geq \outfreethr/|\outset_\prone|$.
% ; otherwise, if $\ell=2$, then it can only be $|\outset_\prtwo|\;>|\outset_\prone|$ and $\|\;\res(\vy_{\measSet\setminus \outset_\prtwo}, \vxx_\prtwo)\;\|_\ell^2 \; < \outfreethr_\prone$, whereas if $\ell=\infty$ and $\nu=\inthr^2/|\outset_\prone|$
\end{theorem}


%\begin{corollary}\label{th:inf-GMC-GTLS-equiv}
%	Consider $\ell=+\infty$ and $\outfreethr=\inthr^2$ in \prone.  Correspondingly, consider $\ell=+\infty$ and $\nu=\inthr^2$ in \prtwo.  Then, eq.~\eqref{eq:equivalency} holds with equality.
%\end{corollary}

% Therefore, \prtwo generally rejects more measurements than \prone.  Indeed, such is the case in the estimation scenario in 
Example~\ref{ex:tls_vs_mts} below provides an intuitive explanation of Theorem~\ref{th:relationship}.
Moreover, it shows that, while {\tls} 
 \red{may reject} more measurements than {\mts}, 
it can lead to more accurate estimates of $\vxxtrue$ since it tends to reject ``biased'' measurements.

\begin{example}[Sometimes, Less is More]\label{ex:tls_vs_mts} Consider an estimation problem where (i) the variable to be estimated is a scalar $x$ with true value 
$\xtrue=0$, (ii) three measurements are available, the inliers $y_1=y_2=0$, and the outlier $y_3=4$, and (iii) 
 the measurement model is $y_i= x+n_i$, for all $i=1,2,3$, where $n_i$ is zero-mean and unit-variance additive Normal noise. 
Also, fix $\inthr=2.58$ 
{in \tls} such that $|n_i|\;\leq \inthr$ with probability $\simeq .99$, and, correspondingly,
$\outfreethr=11.35$ {in \mts} such that $n_1^2+n_2^2+n_3^2\leq \outfreethr$ with probability $\simeq .99$. 
Evidently, at $\xtrue=0$, $\res(y_1,\xtrue)=\res(y_2,\xtrue)=0$ and $\res(y_3,\xtrue)=4$. 

In this toy problem, \mts returns an incorrect estimate: \mts classifies all measurements as inliers for $x=4/3$, since then $\res^2(y_1,x)+\res^2(y_1,x)+\res^2(y_3,x)$ is minimized being equal to $32/3\simeq 10.67$, which is less than $\outfreethr$.

On the other hand, \tls rejects more measurements than \mts but finds the correct estimate: 
\tls returns $x=0$, classifying the third measurement as an outlier.
%, which is indeed less than the minimum value of $\res^2(y_1,x)+\res^2(y_1,x)+\res^2(y_3,x)$, $10.67$, which would be \tls's value if all measurements would be accepted as inliers.

\red{Per Theorem~\ref{th:relationship}, if we had set $\outfreethr=0$  in \mts, since $0$ is the cumulative residual error achieved by \tls for the classified inliers, \mts would have returned the correct estimate.}
\end{example}

Example~\ref{ex:tls_vs_mts} can also be used to showcase that although \tls can reject more measurements than \maxcon, still, it finds the true estimate, whereas \maxcon does not. An extended discussion on the \tls vs.~\maxcon comparison is found in~\cite[Appendix~C]{Yang20arxiv-teaser}.

\optional{All in all, although \prtwo may reject more measurements as outliers than \prone, it may still find a more accurate estimate.  In the example above, this occurs since after rejecting an extra measurement as an outlier, \tls can fit the rest of the measurements more tightly in comparison to \mts.}{}


%%%%% Example with \OUTFREETHR = x times \inthr
%\begin{example}[Sometimes, Less is More]\label{ex:tls_vs_mts} Consider an estimation problem where (i) the variable to be estimated is a scalar $x$ with true value 
%	$\xtrue=0$, (ii) five measurements are available, the inliers $y_1=y_2=y_3=y_4=0$, and the outlier $y_5=4$, and (iii) 
%	the measurement model is $y_i= x+n_i$, for all $i=1,2,3,4,5$, where $n_i$ is zero-mean and unit-variance additive Normal noise. 
%	Also, fix $\inthr=2.58$ 
%	\blue{in \tls} such that $|n_i|\;\leq \inthr$ with probability $\simeq .99$, and, correspondingly,
%	$\outfreethr=5\cdot 2.58=12.9$ 
%	Evidently, at $\xtrue=0$, the residuals are $\res(y_i,\xtrue)=0$, for $i=1,2,3,4,5$, and $\res(y_5,\xtrue)=4$. 
%	
%	In this toy problem, \mts returns an incorrect estimate: \mts classifies all measurements as inliers for $x=4/5$, since then $\sum_{i=1}^4\res^2(y_i,x)+\res^2(y_5,x)$ is minimized, and equals $12.8<\outfreethr$.
%	
%	On the other hand, \tls rejects more measurements than \mts, but finds the correct estimate: 
%%$\res^2(y_1,x)+\res^2(y_2,x)+\res^2(y_3,x)>\outfreethr$ for $x=0$, and, consequently, $x=0$ cannot be a solution to \mts.\footnote{Similarly to \mts, in Example~\ref{ex:tls_vs_mts} \maxcon accepts all measurements as inliers for $x=2$, whereas for $x=0$ it can accept only 2 measurements as inliers; as a result, $x=0$ cannot be a solution to \maxcon.}  In contrast, 
%	\tls returns $x=0$, classifying the fifth measurement as an outlier (for $x=0$, \tls achieves an objective function value equal to $2.58^2$, which is indeed less than the minimum value of $\sum_{i=1}^4\res^2(y_i,x)+\res^2(y_5,x)$, $12.8$, which would be \tls's value if all measurements would be accepted as inliers).
%\end{example}

==> sections/guarantees.tex <==
%!TEX root = ../main.tex

\section{A Posteriori Sub-Optimality Guarantee}
\label{sec:guarantees}

\LC{to be rethought: not informative on inlier set}

\input{sections/fig-perf}

We present the first a posteriori sub-optimality bound for \MTS (Theorem~\ref{th:guarantees}).  We also remark on its quality, by discussing its applicability to any algorithm for \MTS, its $O(1)$ compatibility, and its tightness in simulations (Remark~\ref{rem:quality}).  

To these ends, we use the following notation:
\begin{itemize}
    \item $\selSet^\star$ is an optimal solution to \MTS;
	\item $\res(\selSet)\triangleq \min_{x\in\mathbb{X}} \;\;\sum_{i\in\grSet\setminus \selSet}\; h_i^2(y_i,x)$, where $\selSet$ is a rejected set of measurements; i.e., $\res(\selSet)$ is the minimum residual error given the rejection $\selSet$;
	\item $\res^\star_\maxNumber\triangleq\min_{\selSet\subseteq \grSet, \;|\selSet|\leq \maxNumber} \res(\selSet)$; i.e., $\res^\star_\maxNumber$ is the optimal residual error when at most~$\maxNumber$ measurements are rejected;
	\item $\res^\star\triangleq \res(\selSet^\star)$; i.e., $\res^\star$ is the residual error for the optimal outlier rejection $\selSet^\star$.
\end{itemize}


\begin{theorem}[A posteriori sub-optimality bound]\label{th:guarantees} 
If $\selSet$ is a candidate solution by an algorithm for \MTS, then
%the following bound relates the residual error $\res(\selSet)$ of a candidate solution $\selSet$ with the residual error of an optimal solution that rejects the same number of measurements:
\begin{equation}\label{eq:guarantees}
%\res^\star(|\selSet|)\leq \res(\selSet)\leq \res^\star(|\selSet|)+\apost_\selSet(\res(\emptyset)-\res^\star(|\selSet|)),
\frac{\res(\selSet)-\res^\star_{|\selSet|}}{\res(\emptyset)-\res^\star_{|\selSet|}}\leq \apost_\selSet,
\end{equation}
where 
\begin{equation}\label{eq:bound}
\apost_\selSet\doteq\frac{\res(\selSet)}{\res(\emptyset)-\res(\selSet)}.
\end{equation}
If it is also known that $|\selSet|\; \geq |\selSet^\star|$, then,
\begin{equation}\label{eq:bound_refined}
\frac{\res(\selSet)-\res^\star}{\res(\emptyset)-\res^\star}\leq \apost_\selSet.
\end{equation}
\end{theorem}

Eq.~\eqref{eq:guarantees} quantifies the distance between the residual error at the candidate solution $\selSet$, and 
the residual error at an optimal solution that rejects the same number $|\selSet|$ of measurements. 
Generally, we would like $\res(\selSet)$ and $\res^\star_{|\selSet|}$ to be as close as possible (that is, the candidate solution to be close to the optimal solution of the same cardinality).  Eq.~\eqref{eq:guarantees} indicates exactly that: the closer $\apost_\selSet$ is to $0$, the closer $\res(\selSet)$ is to $\res^\star_{|\selSet|}$.
For example, when $\apost_\selSet=0$, then $\res(\selSet)= \res^\star_{|\selSet|}$, 
i.e., we conclude that the algorithm returned a globally optimal solution (among the ones rejecting $|\selSet|$ measurements).
Moreover, eq.~\eqref{eq:bound_refined} completes the picture by stating that 
 if the algorithm rejects at least as many measurements as the optimal solution ($|\selSet|\; \geq |\selSet^\star|$), then the bound in eq.~\eqref{eq:bound_refined} compares the quality of $\selSet$ directly with the optimal residual error of $\selSet^\star$, the optimal solution of \MTS.


\begin{remark}[Quality of bound]\label{rem:quality}
{The bound is algorithm-agnostic}, and, as such, it applies to any algorithm for \MTS, including \ransac. Also, it is computable in $O(1)$ time, assuming $\res(\emptyset)$ and $\res(\selSet)$ are available upon the algorithm's termination (for example, \name computes $\res(\emptyset)$ at the initialization step, and $\res(\emptyset)$ at the termination step).  Finally, 
we showcase the bound's tightness by considering simulation examples, over \MTS instances of {eq.~\eqref{eq:linear}'s} form.  Specifically,  we generate small instances for which we can compute the optimal solution and 
 evaluate the residual error $\res^\star$.  We compute the optimal solution using CPLEX~\cite{CPLEXwebsite}, a popular library for mixed-integer linear programming, and compare the optimal solution against a candidate solution $\selSet$. 
We find the candidate solutions using the greedy algorithm in~\cite{nemhauser78analysis}.  
%The greedy algorithm, at each iteration, rejects the measurement that induces the largest decrease in the residual error. 
The results are averaged over 10 Monte Carlo simulations, and summarized in Fig.~\ref{fig:perf}.
Fig.~\ref{fig:perf} shows in blue the actual performance of the greedy algorithm (true $(\res(\selSet)-\res^\star)/(\res(\emptyset)-\res^\star)$),
and in red the bound $\apost_{\selSet}$.   Overall, we observe that the bound predicts tightly the actual sub-optimality ratio (note the scale of the $y$-axis), and its quality improves for increasing number of outliers. 
\end{remark}





==> sections/notation.tex <==
%!TEX root = main.tex

\myParagraph{Notation} 
\label{sec:notation}
Calligraphic fonts denote finite countable sets (e.g., $\calA$); and blackboard bold fonts denote any other type of sets (e.g., $\mathbb{R}$ denotes the set of real numbers).
%, and $\mathbb{P}^3$ denotes the projective 3-space). 
Given a set $\calA$, then 
%$2^{\calA}$ denotes the power set of $\calA$; 
$|\calA|$ denotes $\calA$'s cardinality.
%; given another set $\calB$, the set  $\calA\setminus\calB$ denotes set removal, i.e., the set of elements in $\calA$ that are not in~$\calB$. Given a set $\mathcal{V}$, a set function $f:2^\calV\to \mathbb{R}$, and an element $x\in \mathcal{V}$,  then $f(x)$ is a shorthand that denotes $f(\{x\})$.  
% Lowercase letters denote vectors and scalars (e.g.,
% $x$), and uppercase letters denote matrices (e.g., $A$).  
% %Given a matrix $A$, then $A^\top$\! is its transpose; and $\|A\|$ is its norm.  The type of norm ($\ell_0$, $\ell_1$, $\ell_2$, $\infty$, or Frobenius) will be noted with a subscript, when relevant.  
% We end definitions, theorems, etc.~with the symbol $\lrcorner$ to denote the end of their statements.

==> sections/old-alg-GNC.tex <==
%!TEX root = main.tex

\begin{algorithm}[t]\label{alg:gnc}
	\caption{Graduated Non-Convexity for Truncated Least Squares (\gnc-\tls)~\cite{Yang20ral-GNC}.}
	\SetAlgoLined
	\KwIn{\mbox{\tls's input; \gncdisc, \textit{MaxIterations} $\geq 0$.}}
	\KwOut{Indices of measurements classified as inliers.}
	\BlankLine
	{\mbox{$\weights\myat{0} = \bm{1}_\meas;\;\;\vxx\myat{0} = \mathrm{VariableUpdate}(\weights^{0})$\label{line:gnc-initializeStart}\tcp*[l]{\hspace{-0.6em}eq.\hspace{0.2em}\eqref{eq:gncVariableInitilize}}}}
%	 $v^{(0)} = \sumAllPointsIn{\meas}\; w_i^{(0)}\;\res^2(\vy_i,\vxx^{0})$\label{line:gnc-initializeValue}\;
%  $\mu^{(0)}= \left( \frac{2\max_{i\; \in\; \meas}\;\res(\vy_i, \vxx\myat{0}) }{\inlierNoise} -1 \right)^{-1} $
   $\mu^{(0)}=\frac{\inthr^2}{2\max_{i\; \in\; \meas}\;\res^2(\vy_i, \vxx\myat{0})-\inthr^2}$;\quad$\iteration=1$\label{line:gnc-initializeEnd}\;
	\While{$\iteration < \text{MaxIterations}$ {\bf and} $\mathrm{IsNotBinary}(\weights\myat{\iteration-1}$)\label{line:whileStart}}{
  \mbox{$\weights\myat{\iteration} = \mathrm{WeightUpdate}(\vxx\myat{\iteration-1},\mu^{(\iteration-1)}, \inlierNoise)$\label{line:gnc-weightsUpdate}\tcp*[l]{\hspace{-0.6em}eq.\hspace{0.2em}\eqref{eq:weightUpdate}}}\\
  $\vxx\myat{\iteration} = \mathrm{VariableUpdate}(\weights\myat{\iteration})$;\label{line:gnc-variableUpdate}\hspace{.2em}\tcp{\hspace{-0.6em}eq.~\eqref{eq:variableUpdate}}
%	$v^{(\iteration)} = \sumAllPointsIn{\meas}\; w_i^{(\iteration)}\;\res^2(\vy_i,\vxx\myat{\iteration})$\label{line:gnc-valueUpdate}\;
   $\mu^{(\iteration)} = \gncdisc\cdot \mu^{(\iteration-1)}$;
  $\iteration++$\label{line:gnc-muUpdate}\;
	% \lIf{$|v^{(\iteration)}-v^{(\iteration-1)}|\;<\convergthr$}{\KwBreak\label{line:gnc-convergence}}
	}
	\Return $\supp(\bm w\myat{\iteration-1})$.
\end{algorithm}

==> sections/old-relatedWork.tex <==
%!TEX root = ../main.tex

\section{Extended Literature Review}
\label{sec:relatedWork}

\LC{Particularly, recent work has generalized  such costs into a single parametrized function~\cite{Barron19cvpr-adaptRobustLoss} and Chebrolu \etal~\cite{Chebrolu2020arxiv-adaptiveRobustKernels} proposed automatic methods to select the optimal parameter for the problem in hand.}
%whose shape is controlled by the parameter~$\inthr$.}

We extend the literature review in Section~\ref{sec:intro}, across robotics and computer vision (Section~\ref{sec:relatedWork_robotComp}), and statistics and control (Section~\ref{sec:relatedWork_statistics}).
% as well as, across sub-optimality guarantees in outlier-robust estimation (Section~\ref{subsec:relWork_guarantees}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Outlier-robust estimation in robotics and computer vision}\label{sec:relatedWork_robotComp}

Outlier-robust estimation is an active research area in robotics and computer vision for decades~\cite{Meer91ijcv-robustVision,Stewart99siam-robustVision,Bosse17fnt}. 
Traditionally, low-dimensional problems are solved using \ransac~\cite{Chen99pami-ransac} (e.g., 3D registration, and two-view geometry).
\ransac is efficient and effective for low outlier rates~\cite{Speciale17cvpr-consensusMaximization}.  However, the need to cope with higher outlier rates pushed research towards global optimization methods, such as \emph{branch-and-bound} (\BnB)~\cite{Bazin14eccv-robustRelRot,hartley2009ijcv-global,Zheng11cvpr-robustFitting,Li09cvpr-robustFitting,Speciale17cvpr-consensusMaximization}, and \emph{mixed-integer programming} (MIP)~\cite{Chin16cvpr-outlierRejection}.
Nevertheless, for high-dimensional problems (e.g., SLAM), \ransac, \BnB, and MIP are typically  slow to be practical: in the worst-case, they require exponential run-time.  Hence, research has also focused on  M-estimators, in conjunction with either non-convex optimization~\cite{Sunderhauf12iros,Agarwal13icra,Olson12rss}, or convex relaxations~\cite{Lajoie19ral-DCGM}, possibly also including decision variables for the  outlier rejection~\cite{black1996ijcv-unification,Lajoie19ral-DCGM,Sunderhauf12iros,Agarwal13icra}.

In more detail, representative outlier-robust methods for 3D registration, two-view geometry, and SLAM are the following. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myParagraph{Robust 3D registration} 
The goal is to find the transformation (translation and rotation) that aligns two point clouds.
In the presence of outliers, created by incorrect point correspondences, one typically 
resorts to \ransac~\cite{Fischler81,Chen99pami-ransac}, along with a 3-point minimal solver 
---the outlier-free problem admits well-known closed form solutions~\cite{Arun87pami,Horn87josa}.
But when the outliers' number is more than 50\%, \ransac tends to be slow, and brittle~\cite{Speciale17cvpr-consensusMaximization,Bustos18pami-GORE}.  Thereby, recent approaches adopt either robust cost functions~\cite{MacTavish15crv-robustEstimation,Bosse17fnt,Zhou16eccv-fastGlobalRegistration}, or \BnB~\cite{Yang16pami-goicp,Campbell17cvpr-globallyOptRobustTwoView,Bustos18pami-GORE}: Zhou\setal~\cite{Zhou16eccv-fastGlobalRegistration} propose \emph{fast global registration (FGR)}, which is based on the Geman-McClure robust cost function;
Yang\setal~\cite{Yang16pami-goicp} propose a  approach; Campbell\setal~\cite{Campbell17cvpr-globallyOptRobustTwoView} employ \BnB to search the space of camera poses, guaranteeing global optimality without requiring a pose prior;
and Bustos\setal~\cite{Bustos18pami-GORE} add a pre-processing step, that removes gross outliers before \ransac or \BnB.
Other approaches, that iteratively compute point correspondences, include \emph{iterative closest point} (ICP)~\cite{Besl92pami,Segal06rss-generalizedICP},
and \emph{trimmed iterative closest point algorithm}~\cite{Chetverikov05ivc-tICP}; all require an accurate initial guess~\cite{Zhou16eccv-fastGlobalRegistration}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myParagraph{Robust two-view geometry} 
The problem consists in estimating the relative pose (up to scale) between 
two images, given pixel correspondences. In robotics, \ransac is again the go-to approach~\cite{Scaramuzza11ram}, typically in conjunction with
Nister's 5-point method~\cite{Nister03cvpr}, a minimal solver ---other minimal solvers exist when one is given a reference 
direction~\cite{Naroditsky12pami-3point}, the relative rotation~\cite{Kneip11bmvc}, or motion constraints~\cite{Scaramuzza11ijcv}.
In computer vision, recent approaches are investigating the use of provably-robust techniques, typically based on \BnB:
Hartley\setal\cite{hartley2009ijcv-global} propose a \BnB approach for $\ell_\infty$ optimization in one-view and two-view geometry;
Li~\cite{Li09cvpr-robustFitting} uses \BnB and mixed-integer programming for two-view geometry;
Bazin\setal~\cite{Bazin14eccv-robustRelRot} use \BnB for rotation-only estimation;
Chin\setal~\cite{Chin16cvpr-outlierRejection} propose a method to remove outliers in conjunction with mixed-integer linear programming;
Zheng\setal~\cite{Zheng11cvpr-robustFitting} use \BnB to estimate the fundamental matrix;
and Speciale\setal~\cite{Speciale17cvpr-consensusMaximization} improve \BnB approaches by including linear matrix inequalities.
\BnB is typically slow~\cite{Li09cvpr-robustFitting}, but it is able to tolerate high outlier rates.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myParagraph{Robust SLAM}
Outlier-robust SLAM has traditionally relied on M-estimators; e.g.,~\cite{Bosse17fnt}.  
Olson and Agarwal~\cite{Olson12rss} use a max-mixture distribution to approximate multi-modal
measurement noise. 
S\"{u}nderhauf and Protzel~\cite{Sunderhauf12iros,Sunderhauf12icra} augment the problem with latent binary variables responsible for 
deactivating outliers.  Latif~\etal \cite{Latif12rss} propose \emph{realizing, reversing, and recovering} (\rrr), which performs loop-closure outlier rejection, by clustering measurements together and checking for consistency using the chi-square inverse test as an outlier-free bound.  A pair-wise consistency check for multi-robot SLAM, \emph{pair-wise consistency maximization} (\pcm), was proposed by Mangelson~\etal \cite{Mangelson18icra}.
Agarwal \etal~\cite{Agarwal13icra} propose \emph{dynamic covariance scaling} (\dcs), which adjusts the measurement covariances to reduce the influence of outliers.
Lee~\etal~\cite{Lee13iros} use expectation maximization. 
The papers above rely either on the availability of an initial guess for optimization, or on parameter tuning. 
Recent work also includes convex relaxations for outlier-robust SLAM~\cite{Wang13ima,Carlone18ral-robustPGO2D,Arrigoni18cviu,Lajoie19ral-DCGM}. 
Currently,  
only~\cite{Lajoie19ral-DCGM} provides so far 
sub-optimality guarantees, which however degrade with the quality of the relaxation.  Additionally,~\cite{Lajoie19ral-DCGM}  requires parameter tuning.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Outlier-robust estimation in statistics and control}\label{sec:relatedWork_statistics}

Outlier-robust estimation has received long-time attention in statistics and control~\cite{Huber64ams,Kalman60}.  It has a fundamental applications, such as prediction and learning~\cite{Diakonikolas201focs-robustEstimation}, linear decoding~\cite{Candes05tit}, and secure state estimation for control~\cite{Pasqualetti13tac-attackDetection}.  

Outlier-robust estimation in statistics, in its simplest form, aims to learn the mean and covariance of an unknown distribution, given both a portion of \emph{noiseless} i.i.d.~samples, and a portion of arbitrarily corrupted samples (outliers); particularly, the number of outliers is assumed known.\footnote{In contrast, eq.~\eqref{eq:nls}'s framework (and, correspondingly, \MTS's)  considers the estimation of an unknown parameter given some measurements, which framework is equivalent to the estimation of the parameter given non-i.i.d.~samples (the samples depend on the unknown parameter).}
Then, researchers provide polynomial time near-optimal algorithms~\cite{Diakonikolas201focs-robustEstimation, Liu19arxiv-TrimmedHardThresholding}.
 
In scenarios where one aims to estimate an unknown parameter given noisy, and possibly outlying, measurements, then researchers focus on outlier-robust reformulations of eq.~\eqref{eq:nls}.  For example, Rousseeuw~\cite{Rousseeuw11dmkd} proposed a celebrated algorithm to solve a dual reformulation of \MTS, that aims to minimize the residual errors of the remaining measurements given a maximum number of measurement rejections.  The algorithm assumes the outliers' number known, and as such, requires parameter tuning. Similar celebrated algorithms, that also assume the outliers' number known,  are the forward greedy by Nemhauser \etal~\cite{nemhauser78analysis}, and forward-backward greedy by Zhang~\cite{Zhang11tit-ForwardBackGreedy} 
(notably, both algorithms have quadratic run-time, a typically prohibitive run-time for robotics and computer vision applications, such as 3D registration, two-view, and SLAM).
In contrast to~\cite{Rousseeuw11dmkd,nemhauser78analysis,Zhang11tit-ForwardBackGreedy}, the greedy-like algorithm proposed in~\cite{Liu2018tsp-GreedyRobustRegression} considers the outliers' number unknown.  However, it still requires parameter tuning, this time for an outlier-free bound parameter.

Outlier-robust estimation in control takes typically the form of secure state estimation in the presence of outliers (caused by sensor malfunctions, or measurement attacks)~\cite{Pasqualetti13tac-attackDetection,Mishra2017tac-secureStateEstimation,Aghapour2018cdc-outlierAccomodation,Luo19arxiv-SecureStateEst}.  Particularly, in~\cite{Pasqualetti13tac-attackDetection,Mishra2017tac-secureStateEstimation,Aghapour2018cdc-outlierAccomodation,Luo19arxiv-SecureStateEst}, the researchers propose optimal algorithms, that achieve exact state estimation when the non-outlying measurements are noiseless.  However, the algorithms have exponential run-time.

\subsection{Sub-optimality guarantees in outlier-robust estimation}\label{subsec:relWork_guarantees}

Additionally to the aforementioned algorithms that offer sub-optimality guarantees (or certificates of optimality), researchers have also provided conditions for exact estimation when some of the measurements are outliers, while the rest are noiseless~\cite{Candes05tit,Zhang11tit-ForwardBackGreedy}. However, the conditions' evaluation is NP-hard.  Additionally, the conditions are restricted on a linear and convex framework, where the measurements are linear in the unknown parameter $x$, and $x \in \mathbb{R}^n$.\footnote{In contrast, Section~\ref{sec:guarantees} provides a posteriori sub-optimality bounds, computable in $O(1)$ run-time, and applicable to even non-convex and non-linear frameworks, such as for 3D registration, two-view geometry, and SLAM.}

==> sections/problem-formulation.tex <==
%!TEX root = main.tex

\section{Outlier Rejection: a Minimally Trimmed Squares Formulation}
\label{sec:problem_formulation}

\begin{example}[Robust linear estimation and bound $\perfBudgMin_{\grSet\setminus \selSet}$]\label{ex:linear_dec} 
In linear estimation one wishes to recover a parameter $x \in \mathbb{R}^n$ from a set of noisy measurements $y_i=a_i^\top x+d_i$, $i\in \grSet$, where $a_i$ is a known vector, and 
 $d_i \in \Real{}$ models the unknown measurement noise.
 Some of the measurements (the inliers) are such that the corresponding noise $d_i$ can be assumed to follow a Gaussian distribution, while others (the outliers) may be affected by large noise. 
 Therefore, our \MTS estimator can be written as:  
 %
\begin{equation}\label{eq:dual_linear_regr}
\min_{x\in \mathbb{R}^n} \;\; \min_{\selSet\subseteq \grSet} \;\;\;|\selSet|,\;\;\text{s.t.}\;\;\;\sum_{i \in \grSet\setminus\selSet} \|y_i-a_i^\top x\|^2\;\leq \perfBudgMin_{\grSet\setminus \selSet}.
\end{equation}
%
Evidently, $\perfBudgMin_{\grSet\setminus \selSet}$ 
must increase with the number of inliers, since each inlier adds a positive summand $\|y_i-a_i^\top x\|^2$ due to the presence of noise. 
Moreover, since the sum is restricted to the inliers, for which the noise is assumed to be Gaussian, we can compute the desired outlier-free bound explicitly: 
if 
$d_i$ follows a Gaussian distribution, then each $\|y_i-a_i^\top x\|^2_{2}$ follows a $\chi^2$ distribution with $1$ degree of freedom. %, since $y_i=A_i^\top x+d_i$. 
 Thus, with desired probability $p_\epsilon$ (e.g., $0.99$),  $\|y_i-a_i^\top x\|^2_{2}\leq \perfBudgMin$ where $\perfBudgMin$ is the $p_\epsilon$-quantile of the $\chi^2$ distribution, 
 and  the outlier-free bound is $\perfBudgMin_{\grSet\setminus \selSet}=|\grSet\setminus \selSet| \perfBudgMin$.
\hfill $\lrcorner$
\end{example}

\begin{remark}[Generality \!and \!applicability]
In this paper we address robustness in non-linear and non-convex estimation problems 
as the ones arising in robotics and computer vision. 
Therefore, while the linear estimation Example~\ref{ex:linear_dec} is instructive 
 (and indeed we will prove in Section~\ref{sec:hardness} that even in such a simple case, it is not possible to even approximate the \MTS 
estimator in polynomial time), the algorithms and bounds presented in this paper hold for any 
function $h_i(y_i,x)$ and  any domain $\mathbb{X}$. 
In contrast with related work~\cite{Rousseeuw11dmkd, Yang16pami-goicp}, we do not assume the number of outliers to be known in advance (an unrealistic assumption in perception problems). 
Indeed, our \MTS formulation looks for the smallest set of outliers. 
% This is significant from an application standpoint, where the number of outliers is unknown.  
Finally, while the formulation~\eqref{eq:MTS} requires to set an outlier-free threshold, we will propose an algorithm (Section~\ref{sec:algorithms}) that will automatically compute a suitable threshold without any prior knowledge about the measurement noise. 
% The proposed algorithm, \nameLong (\name), only requires the availability of a black-box solver for the 
% outlier-free problem in eq.~\eqref{eq:nls}.
\hfill $\lrcorner$
%the proposed algorithm (Section~\ref{sec:algorithms}) only requires 
%as we will discuss in  
\end{remark}


In summary, \MTS is a general non-linear and non-convex outlier rejection framework.
We exemplify its generality by discussing its application to three core perception problems:
 3D registration, two-view geometry, and SLAM.

==> sections/supp_2-view.tex <==
%!TEX root = supplemental.tex
\newpage
\clearpage
\subsection{Supplemental for  Robust Two-view Geometry}
\label{sec:supp_view}

\input{supp_fig-2view}

==> sections/tab-parameters.tex <==
%!TEX root = ../main.tex

\begin{table}[h]
  \centering\footnotesize
\setlength{\tabcolsep}{4pt}
\setlength{\extrarowheight}{3pt}
\begin{tabular}{lccc}\toprule
\emph{Application} & \emph{\convergthr} & \noiselowbound & \noiseupbound \\
\midrule
\scenario{Mesh Registration} & \num{1e-4} & $\noiselowboundMesh$ & $\noiseupboundMesh$\\
\scenario{Shape Alignment} & \num{1e-4} & $\noiselowboundShape$ & $\noiseupboundShape$\\
\scenario{PGO} & \num{1e-4} & $\noiselowboundPGO$ & $\noiseupboundPGO$\\
\bottomrule\hline
\end{tabular}
\caption{Parameters for \adaptfree (\convergthr) and \gncfree (\noiselowbound and \noiseupbound). 
The $\chi^2$'s {degree of freedom $d$ is equal to $3$ for 2D \PGO and to $6$ for 3D \PGO}.}\label{table:params_auto}
\vspace{-8mm}
\end{table}

